"Project smells" -- Experiences in Analysing the Software Quality of ML Projects with mllint

Machine Learning (ML) projects incur novel challenges in their development and productionisation over traditional software applications, though established principles and best practices in ensuring the project's software quality still apply. While using static analysis to catch code smells has been shown to improve software quality attributes, it is only a small piece of the software quality puzzle, especially in the case of ML projects given their additional challenges and lower degree of Software Engineering (SE) experience in the data scientists that develop them. We introduce the novel concept of project smells which consider deficits in project management as a more holistic perspective on software quality in ML projects. An open-source static analysis tool mllint was also implemented to help detect and mitigate these. Our research evaluates this novel concept of project smells in the industrial context of ING, a global bank and large software- and data-intensive organisation. We also investigate the perceived importance of these project smells for proof-of-concept versus production-ready ML projects, as well as the perceived obstructions and benefits to using static analysis tools such as mllint. Our findings indicate a need for context-aware static analysis tools, that fit the needs of the project at its current stage of development, while requiring minimal configuration effort from the user.

==> papers.tex <==
%%
%% This file is basically a scratchpad for writing down information, quotes and whatever else can be extracted out of papers that I've read / find important for this ICSE-SEIP paper.
\cite{sculley2015hidden}
- One of the first papers to analyse risk factors in developing ML applications through the lens of technical debt.
- Mentions Configuration Debt: tech debt in configuring tools, e.g. linters

\cite{muralidhar2021mlops-antipatterns}
"MLOps -Machine Learning Operations- refers to the body of work that focuses on the full lifecycle of ML model deployment, performance tracking, and ensuring stability in production pipelines" (introduction)
Antipatterns:
- Data Leakage: broadly refers to situations where the model uses information that it is not supposed to have, or will not be available in production. Leads to overly optimistic performance estimates and poses serious downstream problems upon model deployment.
- Act Now, Reflect Never: i.e. deploy and forget. Refers to production-deployed ML systems that are not being monitored, tracked and debugged. Can lead to 1) concept drift or 2) irrelevant or easily recognisable erroneous predictions or 3) adversarial attacks.
- Tuning-under-the-Carpet: hyper-parameters are important, so they should be tuned correctly and, moreover, the process by which they are tuned should be explicit, well-documented, reproducible and easily adaptable.
- PEST (Perceived Empirical SuperioriTy): sometimes, novel contributions to applied ML seem to show better performance in their empirical verification, but are not necessarily always better than properly tuned existing methodologies. Sometimes, older methods / ML model architectures outperform more recent and sophisticated model architectures, simply by appropriately tuning hyperparameters. KISS.
- Bad Credit Assignment: refers to the failure to appropriately identify the source of performance gains in a modeling pipeline. E.g. for a new model with better empirical performance, the improved performance is attributed to the new model, while the improvement could instead also come from clever problem formulations, data preprocessing, hyper-parameter tuning, or other variables outside of the new model (or even a combination of all the above).
- Grade-your-own-Exam: basically refers to never truly evaluating your model, except for using a test set that is already known during model development. Much like students who memorise the final exam questions, this causes the model to perform optimistically well in training and testing, but fails to achieve the same performance in production with real data.
- Set & Forget: basically refers to concept drift: when statistical properties of the target variable that the learning model is trying to predict, change over time.
- Communicate with Ambivalence: ML model should be able to communicate about the certainty / uncertainty of it's predictions. something about a Brier score?
- Data Crisis as a Service: refers to failure to record the process for preparing and sanitising the data. Not being able to reproduce your data cleaning and preparation processes with new data means re-learning your model may end up with vastly different results.
---
- Recommends: using assertions to track data quality, which is crucial since ML models can be very dependent on faulty or noisy data. Suitable checks and balances on data across the enterprise can ensure a safe operating environment for ML algorithms.
- Document your data lineage, cleaning etc. so models can be situated back in time and in specific data slices for re-training or re-tuning --> implies reproducibility
- no. 4 is basically a recommendation to use versioning for your models.
- ensure human in the loop at multiple levels.

\cite{washizaki2019se-patterns}
"Thus, we set out to collect good/bad SE design patterns for ML techniques to provide developers with a comprehensive and ordered classification of such patterns. We report here preliminary results of a systematic-literature review (SLR) of good/bad design patterns for ML."
- Contains 33 design patterns and anti-patterns from literature (18) as well as grey literature (15), e.g. Google's Rules for ML.
- Most patterns deal with model deployment
- 

\cite{kriens2019software}
- Writing code is one thing, industrialising it is a whole other thing.
- Traditionally has been difficult in SE, but has in the mean time been solved with package registries and package managers, Docker, binary distributables.
- Proposes the idea of an OSGi-like model for distributing ML models
- "In OSGi, modules never depend on other modules, they depend on APIs"
- The OSGi therefore took the innovative step to abstract dependency types into the Requirements and Capabilities specification. This specification defines how generic capabilities and requirements are encoded and allows almost anything that a developer can make assumptions about to be specified as a requirement on capabilities so that it can be verified by tools.
- For ML models, this could include what the model accepts as input (e.g. only images 256x256 pixels), what the model accepts as output or what dataset the model was trained on.
- "This urges for a new packaging model for ML models that captures all necessary metadata to automate the assembly process"

\cite{kiraly2021scitype}
- Proposes a new type system based on scientific types to better capture the meaning of common elements in ML workflows based on the set of operations that we usually perform with them (i.e. their interface) and their statistical properties.
- Favours OOP for developing ML libraries / toolkits
- Primarily about library architecture and design, not very interesting for ML applications

\cite{google2017production-rubric}
- Presents 28 specific tests and monitoring needs for production-grade ML systems, drawn from Google's experience with a wide range of production ML systems.
- ML reliability becoming increasingly critical
- "One way to see this is to consider ML training as analogous to compilation, where the source is both code and training data. By that analogy, training data needs testing like code, and a trained ML model needs production practices like a binary does, such as debuggability, rollbacks and monitoring."
- Also presents a way to calculate a score from the adherence to each of the best practices below.
---
- Features & data
    - capture training data in a schema --> GreatExpectations
    - make sure all features are beneficial
    - make sure no feature's cost is too much
    - programmatically enforce meta-level requirements on features, e.g. prohibit the use of user-specific data such as age, prohibit deprecated features. --> GreatExpectations
    - ensure privacy
    - ensure features can be added quickly
    - ensure all feature creation code is tested properly. --> GreatExpectations + other automated tests + possibly DVC
- ML model development
    - do code reviews on every model
    - offline & online metric s should correllate correctly --> A/B testing
    - all hyperparameters have been tuned
    - impact of model staleness is known: what is the impact of using last month's model instead of this month's model? --> A/B testing
    - ensure that a simpler model doesn't outperform your more sophisticated implemetation
    - model quality is sufficient on all important data slices --> i.e. don't just test your model performance on all data, but take some important subsets of the data too, e.g. per country.
    - model has been tested for considerations of inclusion --> ML fairness
- ML infrastructure
    - Training is reproducible --> DVC
    - Model specification code is unit tested --> unit tests, even if only with miniature training data to verify that configuration is correct and works.
    - Full ML pipeline is integration tested -->  there must be a fully automated test that runs regularly and exercises the entire pipeline, validating that data and code can successfully move through each stage and that the resulting model performs well. --> testing, possibly with DVC's CI for ML solution stuff.
    - Model quality is evaluated before attempting to serve it (i.e. test it before you allow users to use it)
    - Model allows debugging by observing the step-by-step computation of training or inference of a single sample. --> TensorFlow debugger: https://www.tensorflow.org/tensorboard/debugger\_v2
    - Models are tested via a canary process before they enter production serving environments
    - Models can be quickly and safely rolled back to a previous serving version --> version your data, code and, particularly, models. Then use good deployment strategy, e.g. Kubernetes and https://github.com/SeldonIO/seldon-core or MLFlow or something similar.
- Monitoring ML
    - Data invariants hold in training and in serving inputs --> make e.g. GreatExpectations input data quality testing also part of your API methods?
    - Training and serving features compute the same values
    - Models are not too stale
    - The model is numerically stable
    - The model has not experienced a dramatic or slow-leak regressions in training speed, serving latency, throughput, or RAM usage --> e.g. use SeldonCore and Grafana / Prometheus to monitor speed and performance
    - The model has not experienced a regression in prediction quality on served data

\cite{washizaki2019se-patterns}

\cite{nascimento2020se4ml-slr}
- SLR of SE for ML / AI techniques & best practices
- 

\cite{zhang2020ml-testing}
- SLR about testing ML systems.
- It covers 138 papers on testing properties (e.g., correctness, robustness, and fairness), testing components (e.g., the data, learning program, and framework), testing workflow (e.g., test generation and test evaluation), and application scenarios (e.g., autonomous driving, machine translation). The paper also analyses trends concerning datasets, research trends, and research focus, concluding with research challenges and promising research directions in machine learning testing.

\cite{xu2015too-much-configuration}
1. Hide or remove configuration parameters that are seldom set by any user. This requires to build
user-feedback loops for configuration settings. Finding 1(a) § 3.1
2. Promote parameters set by most users to be the “first-class” ones. Include them in tutorials and
guidebooks to let users focus on these parameters first. Finding 1(b) § 3.1
3. If possible, convert numeric parameters into enumerative or Boolean types with expressive,
representative values to make the settings simple for users.
Finding 2(a) § 3.2
4. Avoid enumerative parameters with too many options. Five options should be sufficient in terms
of user flexibility. Finding 2(b) § 3.2
5. Only expose the configuration parameters with explicit semantics and/or visible external system
impact. Finding 4 § 3.

\cite{serban2020se4ml-adoption}
"Our findings indicate, for example, that larger teams tend to adopt more practices, and that traditional software engineering practices tend to have lower adoption than ML specific practices"

